Augmenting Teamwork through AI Agents as Spatial Collaborators

As Augmented Reality (AR) and Artificial Intelligence (AI) continue to converge, new opportunities emerge for AI agents to actively support human collaboration in immersive environments. While prior research has primarily focused on dyadic human-AI interactions, less attention has been given to Human-AI Teams (HATs) in AR, where AI acts as an adaptive teammate rather than a static tool. This position paper takes the perspective of team dynamics and work organization to propose that AI agents in AR should not only interact with individuals but also recognize and respond to team-level needs in real time. We argue that spatially aware AI agents should dynamically generate the resources necessary for effective collaboration, such as virtual blackboards for brainstorming, mental map models for shared understanding, and memory recall of spatial configurations to enhance knowledge retention and task coordination. This approach moves beyond predefined AI assistance toward context-driven AI interventions that optimize team performance and decision-making.

==> Sections/02_Team.tex <==
%\section{Humans-AI Team in AR }
%Teams consist of two or more individuals collaborating to achieve a shared objective \cite{salas2000teamwork}. As the foundation of organizational work, teams coordinate efforts to tackle complex tasks, demonstrating interdependencies in workflows, goals, and outcomes that reflect their collective responsibility \cite{kozlowski2006enhancing, gomez2020taxonomy, baron2003group}.  
%Human-AI Teams (HATs) consist of two or more individuals working with at least one AI agent \cite{}, integrating agent ai as an active teammate capable of assisting, coordinating, and adapting in collaborative tasks \cite{}.


%\section{Design of AI agents in AR}
%Unlike traditional interfaces, Augmented Reality (AR) provides a hands-free, immersive environment where AI agents can function as spatially aware entities, interacting with users in real-time, real-world contexts. AR interfaces typically rely on gestures, gaze tracking, and speech for interaction, as seen in devices like the Microsoft HoloLens, which employs gaze-based selection and speech-driven AI assistance, or Meta Orion, which promises ubiquitous interaction, aiming to replace conventional screen-based interfaces with more intuitive, context-aware AI interactions.

% In this work, we propose leveraging AR’s spatial computing capabilities—particularly its real-time environmental understanding—in combination with team dynamics analysis to create AI agents that enhance team meetings. These AI agents will act as active collaborators by dynamically generating and adapting supplemental materials to improve communication, coordination, and shared understanding. For instance, AI agents could create virtual blackboards for brainstorming, real-time subtitles to enhance accessibility, or on-demand 3D models to help teams visualize complex concepts. By augmenting mental models and adapting to team needs in real time, these AI agents can bridge gaps in understanding, facilitate problem-solving, and enhance collaborative decision-making in immersive AR environments.

% Building on prior research that has recognized the challenges of virtual meeting, in person and immerse we propose to deepen the discussion to AR environments and respond to the following questions 
% \begin{itemize}
%     \item RQ1: What are the optimal design for AI assistants in AR that enhance usability, interaction, and effective team collaboration?
%     \item RQ2: What are the spatial and proxemic factors in AR that sould be consider to enhance 
%     \item RQ3: What should be the emboidement representation of the ai-agents focus on team rather than interpersonal factors?
%     \item RQ4: When and how should ai-agents intervene in team workflows within AR? How can it detect when users need assistance without disrupting collaboration?
% \end{itemize}


% Real-World-Oriented AI Agents
% The driving force behind Artificial Intelligence (AI) research from its inception has been the pursuit of intelligence that matches or surpasses human capabilities \cite{haenlein2019brief, turing2009computing, fox2014current}. The significant advancements of AI over the past decades have been driven by deep learning algorithms \cite{aggarwal2022has}, more powerful and compact hardware \cite{haas2019s, zaman2021custom}, and access to extensive datasets for training \cite{xie2024frontiers}.

% Among the most prominent outcomes of these advancements is the rise of Large Language Models (LLMs) \cite{zhao2023survey}, which have revolutionized natural language understanding and multimodal processing \cite{zhang2024mm, chang2024survey}. Models such as Google’s Gemini \cite{team2023gemini}, OpenAI’s ChatGPT \cite{achiam2023gpt}, and Meta’s LLaMA \cite{dubey2024llama} exemplify how AI has progressed toward more context-aware, reasoning-capable systems. These developments have not only advanced new human-computer interactions but have also have established a foundation for AI agents capable of human-like behaviour, cognitive processing, logical reasoning and independent problem solving \cite{park2023generative, chen2024towards, gizzi2022creative}. As a result, extensive research has evaluated AI agents’ ability to perform these tasks at a level comparable to humans, with studies demonstrating promising results in creative generation, planning, and design \cite{}.



% In response, XR researchers emphasize the need to design AI agents that are immersed in the real world, capable of observing, interacting with, and continuously learning from their environment and human collaborators in a dynamic and adaptive way. One emerging application of this approach is LLM-based Non-Player Character (NPC) agents, which have been deployed in immersive environments across various fields, including video games, training simulations, and virtual collaboration spaces. These AI-driven agents enhance user engagement by facilitating interaction, adapting to real-time input, and contributing to the collaborative experience \cite{}.

% As collaboration in immersive environments continues to grow, team meetings remain a crucial aspect of organizations for coordination, discussion, and decision-making \cite{}. AI-driven technologies have emerged to enhance team dynamics, improving inclusivity, usability, and overall experience. However, much of this research has focused on dyadic interactions, where AI engages with individuals rather than supporting multi-user team dynamics in virtual meetings. To advance AI agents in immersive environments, it is essential to design systems that go beyond one-on-one interactions and address team behaviors, coordination patterns, and collective needs. We see an opportunity to introduce real-time AI agents in AR-powered virtual meetings, enabling them to adapt to team dynamics, respond to real-world challenges, and leverage the unique affordances of this technology.



% These technologies are redefining how teams communicate and collaborate while also facilitating the integration of AI agents into team meetings, improving coordination, decision-making, and shared understanding through the blend of the digital and physical worlds.





% Emerging studies suggest that immersive technologies, such as AR, VR, and MR, have the potential to mitigate team challenges such as poor engagement, lack of shared understanding team cohesion, and the complexities of geographically distributed teams, which are prevalent in both in-person collaboration and traditional virtual meetings such as Zoom \cite{fernandez2025breaking}.



==> Sections/03_AI_Collaborator.tex <==
% \section{Conclusion and Future Work}
% This position paper takes the perspective of team dynamics and work organization to explore the convergence of AR’s spatial awareness and AI agents' real-time understanding. We propose that AI agents in AR should actively recognize and respond to team needs, dynamically generating the resources required to enhance collaboration. Rather than functioning as passive assistants, these AI agents should act as adaptive facilitators, capable of identifying when a blackboard is needed for brainstorming, generating mental map models for conceptual alignment, or recalling spatial configurations to support knowledge retention and task continuity.

% By shifting the role of AI agents from predefined tools to responsive, context-aware teammates, we can unlock new possibilities for collaborative intelligence in AR environments. Addressing the research questions posed in this paper will be essential to designing AI agents that seamlessly integrate into team workflows, optimize interaction in immersive spaces, and ultimately enhance team performance and decision-making. Through this discussion, we aim to advance the understanding of AI in AR not just as an interface, but as an active enabler of human collaboration.


